Improving Feature Stability during Upsampling -- Spectral Artifacts and the Importance of Spatial Context

Pixel-wise predictions are required in a wide variety of tasks such as image restoration, image segmentation, or disparity estimation. Common models involve several stages of data resampling, in which the resolution of feature maps is first reduced to aggregate information and then increased to generate a high-resolution output. Previous works have shown that resampling operations are subject to artifacts such as aliasing. During downsampling, aliases have been shown to compromise the prediction stability of image classifiers. During upsampling, they have been leveraged to detect generated content. Yet, the effect of aliases during upsampling has not yet been discussed w.r.t. the stability and robustness of pixel-wise predictions. While falling under the same term (aliasing), the challenges for correct upsampling in neural networks differ significantly from those during downsampling: when downsampling, some high frequencies can not be correctly represented and have to be removed to avoid aliases. However, when upsampling for pixel-wise predictions, we actually require the model to restore such high frequencies that can not be encoded in lower resolutions. The application of findings from signal processing is therefore a necessary but not a sufficient condition to achieve the desirable output. In contrast, we find that the availability of large spatial context during upsampling allows to provide stable, high-quality pixel-wise predictions, even when fully learning all filter weights.

==> eccv_2024/figures/exp_seg_example.tex <==
\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.81\textwidth]{eccv_2024/figures/experiments/segmentation/feature maps segmentation.png}
	\caption[]{Comparing predictions and feature maps of the penultimate layer from baseline model (2x2 kernel for upsampling) and model with 11 x 11 kernels for transposed convolution for one test image. 
	We show the full feature maps from the baseline model (left) and large kernel transposed convolution model (right) in supplementary material. The image in top centre is the ground truth segmentation mask. %\Cref{fig:appendix:segmentation:feature:baseline:aeroplane} and \Cref{fig:appendix:segmentation:feature:trans_11_3:aeroplane} respectively
	In the cropped feature map from the baseline, especially in the right channel, a lot of grid like structures are appearing. % that while it is trying to segment out the object in the given input image. 
	These are the grid artifacts. We observe in feature maps from the model with 11 x 11 kernel with a 3x3 kernel in parallel, these grid artifacts are much less present, and when present are smoothed out, making the upsampled feature map look more continuous than grid-like.
	}
	\label{fig:exp:segmentation:comparing_pred_features}
	\end{center}
	\vspace{-1em}
\end{figure*}

==> eccv_2024/figures/feature_maps_teaser.tex <==
\begin{figure}[!ht]
	%\begin{center}
 \begin{tabular}{@{}r@{\hspace{0.5cm}}l@{}}
\scriptsize
\scriptsize Ground truth segmentation overlay&\scriptsize Baseline feature maps, $2\times 2$ kernel.\\
	%\includegraphics[width=0.79\linewidth]{eccv_2024/figures/teaser/iccv23 feature maps segmentation.drawio.pdf}
     %\includegraphics[width=0.3\linewidth]{eccv_2024/figures/teaser/iccv23_gt_segmentation.pdf} 
     \includegraphics[width=0.39\linewidth]{eccv_2024/figures/teaser/iccv23_teaser_gt.pdf} 
 %   Ground truth segmentation mask\\
 %   \vspace{0.5em}
   & \includegraphics[width=0.5\linewidth]{eccv_2024/figures/teaser/iccv23_baseline_feature_maps_segmentation.pdf} \\
   \scriptsize Cropped ground truth &\scriptsize feature maps, $11\times 11+3\times 3$ kernel.\\
 %   Crop showing 2 channels in the feature maps from the baseline\\
 %   \vspace{0.5em}
    \includegraphics[width=0.25\linewidth]{eccv_2024/figures/teaser/iccv2.png} 
   & \includegraphics[width=0.5\linewidth]{eccv_2024/figures/teaser/iccv23_11x11_feature_maps_segmentation2.pdf}
  %  & \scriptsize crop from two feature map channels
    %Crop showing 2 channels in the feature maps from the 11x11 kernel\\
    %\vspace{0.5em}
    %\includegraphics[width=0.5\linewidth]{eccv_2024/figures/teaser/iccv23_17x17_crops_feature_maps_segmentatio.pdf}\\
    %Crop showing 2 channels in the feature maps from the 17x17 kernel}
    %\vspace{0.5em}
     \end{tabular}
  %   \end{center}
	\caption[]{Comparing feature maps of the penultimate layer (before the class predictions) from a baseline model~($2\times 2$ kernel for upsampling, top right) and our model with larger kernels~($11\times 11$ with parallel $3\times 3$, bottom right) for transposed convolutions. While the baseline feature maps miss out on many details and show severe grid artifacts, these artifacts are significantly reduced when larger kernels are used.
 See \cref{subsubsec:exp:setup:segment} for the full feature maps. 
	%We show the full feature maps from the baseline model (middle) and large kernel transposed convolution model (bottom) in supplementary material. 
    %The image in top is the ground truth segmentation mask. %\Cref{fig:appendix:segmentation:feature:baseline:aeroplane} and \Cref{fig:appendix:segmentation:feature:trans_11_3:aeroplane} respectively
	%In the cropped feature map from the baseline, especially in the right channel, a lot of grid like structures are appearing. % that while it is trying to segment out the object in the given input image. 
	%These are the grid artifacts.
    %However, these grid artifacts reduce when using a larger kernel for upsampling~(bottom).
	}
	\label{fig:exp:segmentation:comparing_pred_features}
	
	\vspace{-1.5em}
\end{figure}
%
%
%
%
%
%
\iffalse
\begin{figure}[!ht]
	\begin{center}
 \tiny{
	%\includegraphics[width=0.79\linewidth]{eccv_2024/figures/teaser/iccv23 feature maps segmentation.drawio.pdf}
    \includegraphics[width=0.5\linewidth]{eccv_2024/figures/teaser/iccv23_gt_segmentation.pdf}\\
    Ground truth segmentation mask\\
    \vspace{0.5em}
    \includegraphics[width=0.5\linewidth]{eccv_2024/figures/teaser/iccv23_baseline_feature_maps_segmentation.pdf} \\
    Crop showing 2 channels in the feature maps from the baseline\\
    \vspace{0.5em}
    \includegraphics[width=0.5\linewidth]{eccv_2024/figures/teaser/iccv23_11x11_feature_maps_segmentation.pdf}\\
    Crop showing 2 channels in the feature maps from the 11x11 kernel\\
    \vspace{0.5em}
    \includegraphics[width=0.5\linewidth]{eccv_2024/figures/teaser/iccv23_17x17_crops_feature_maps_segmentatio.pdf}\\
    Crop showing 2 channels in the feature maps from the 17x17 kernel}
    \vspace{0.5em}
	\caption[]{Comparing predictions and feature maps of the penultimate layer from baseline model~(2x2 kernel for upsampling, in middle) and model with larger kernels~(11x11, bottom) for transposed convolution for one test image. 
    We show the full feature maps in supplementary material. 
	%We show the full feature maps from the baseline model (middle) and large kernel transposed convolution model (bottom) in supplementary material. 
    The image in top is the ground truth segmentation mask. %\Cref{fig:appendix:segmentation:feature:baseline:aeroplane} and \Cref{fig:appendix:segmentation:feature:trans_11_3:aeroplane} respectively
	In the cropped feature map from the baseline, especially in the right channel, a lot of grid like structures are appearing. % that while it is trying to segment out the object in the given input image. 
	These are the grid artifacts.
    However, these grid artifacts reduce when using a larger kernel for upsampling~(bottom).
	}
	\label{fig:exp:segmentation:comparing_pred_features}
	\end{center}
	\vspace{-2.5em}
\end{figure}
\fi

==> eccv_2024/figures/fig_transpose_conv_plots.tex <==
\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ResNet Style 3×3_transpose_conv_+3x3.pdf}
	\caption[]{ResNet Style 3×3 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ConvNeXt style 7×7_transpose_conv_+3x3.pdf}
	\caption[]{ConvNeXt style 7×7 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}

\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ConvNeXt style 11×11_transpose_conv_+3x3.pdf}
	\caption[]{ConvNeXt style 11×11 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ConvNeXt style 11×11 + 3×3_transpose_conv_+3x3.pdf}
	\caption[]{ConvNeXt style 11×11 +3x3 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}

==> eccv_2024/figures/fig_transpose_conv_plots_mean.tex <==
\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ResNet Style 3×3_mean_transpose_conv_+3x3.pdf}
	\caption[]{ResNet Style 3×3 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ConvNeXt style 7×7_mean_transpose_conv_+3x3.pdf}
	\caption[]{ConvNeXt style 7×7 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}

\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ConvNeXt style 11×11_mean_transpose_conv_+3x3.pdf}
	\caption[]{ConvNeXt style 11×11 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ConvNeXt style 11×11 + 3×3_mean_transpose_conv_+3x3.pdf}
	\caption[]{ConvNeXt style 11×11 +3x3 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}

==> eccv_2024/figures/fig_transpose_conv_plots_only3x3.tex <==
\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ResNet Style 3×3_transpose_conv_only+3x3.pdf}
	\caption[]{ResNet Style 3×3 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ConvNeXt style 7×7_transpose_conv_only+3x3.pdf}
	\caption[]{ConvNeXt style 7×7 ONLY +3x3
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}

\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ConvNeXt style 11×11_transpose_conv_only+3x3.pdf}
	\caption[]{ConvNeXt style 11×11 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/ConvNeXt style 11×11 + 3×3_transpose_conv_only+3x3.pdf}
	\caption[]{ConvNeXt style 11×11 +3x3 TODO
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}

==> eccv_2024/figures/method_upsampling_abstract.tex <==
\begin{figure}[t]
	\begin{center}
	\includegraphics[width=0.6\linewidth]{eccv_2024/figures/method/upsampling_abstract4.pdf}
	\caption[]{Exchanged kernels in transposed convolution for upsampling. Instead of small~(2$\times$2 or 3$\times$3) transpose convolutions we either use 7$\times$7 or 11$\times$11 with a parallel 3$\times$3 transpose convolutions. 
 These correspond to the operations along {\color{BrickRed} red arrows} in Figure~\ref{fig:unet_plus_block}.}
	\label{fig:upsampling}
	\end{center}
	\vspace{-1em}
\end{figure}

==> eccv_2024/figures/transpose_conv_plots.tex <==
\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=0.98\linewidth]{eccv_2024/figures/experiments/segmentation/transpose_conv_normalized2x2+3.pdf}
	\caption[]{Comparison of performance of different sizes of transpose convolutions from standard sizes like $2\times2$ as well as very large $31\times31$ kernels.All have a parallel 3×3 kernel, as shown in \Cref{fig:unet_plus_block} (bottom left). As backbone a ConvNeXt style 11×11 +3x3 sytle is used. \textcolor{red}{WRITE MORE}
	}\label{fig:transpose_conv_plots}
	\end{center}
	\vspace{-1em}
\end{figure*}

==> eccv_2024/instruction.tex <==
\section{Introduction}
\label{sec:intro}

This document serves as an example submission to ECCV \ECCVyear{}.
It illustrates the format authors must follow when submitting a paper. 
At the same time, it gives details on various aspects of paper submission, including preservation of anonymity and how to deal with dual submissions.
We advise authors to read this document carefully.

The document is based on Springer LNCS instructions as well as on ECCV policies, as established over the years.

\section{Initial Submission}

\subsection{Language}
All manuscripts must be in English.


\subsection{Template}
Papers must be prepared with the official LNCS style from Springer.
This applies to both review and camera-ready versions.
Springer requires manuscripts to be prepared in \LaTeX{} (strongly encouraged) or Microsoft Word. 

Authors preparing their paper with \LaTeX{} must use the template provided by ECCV, which is based on the corresponding Springer class file \texttt{llncs.cls} but includes line numbers for review (\cref{sec:line-numbering}) and properly anonymizes the paper for review (as in this example document).
Authors who -- for whatever reason -- cannot use \LaTeX{} can alternatively use the official LNCS Word template from Springer.
However, it is the authors' responsibility to ensure that the resulting PDF file is consistent with this example paper and follows it as closely as possible (\ie, includes line numbers, is properly anonymized, \etc).

We would like to stress that the class/style files and the template must not be manipulated and that the guidelines regarding font sizes and format must be adhered to. 
For example, please refrain from using any \LaTeX{} or \TeX{} command that modifies the layout settings of the template (\eg, \verb+\textheight+, \verb+\vspace+, \verb+\baselinestretch+, \etc).
Such manual layout adjustments should be limited to very exceptional cases.
This is to ensure that the end product is as homogeneous as possible.

Papers that differ significantly from the required style may be rejected without review.


\subsubsection{Fonts.}
Springer's templates for \LaTeX{} are based on CMR, and the XML templates for Word are based on Times. 
We ask you to use the font according to the template used for your papers. 
Specifically, please refrain from using Times when preparing your paper with \LaTeX{}.
Using a different font can be interpreted as purposely circumventing the length limitations and may lead to rejection without review.


\subsection{Paper Length}
Papers submitted for review must be complete. 
The length should match that intended for final publication. 
Papers accepted for the conference will be allocated 14 pages (plus additional pages for references) in the proceedings. 
Note that the allocated 14 pages do not include the references. 
The reason for this policy is that we do not want authors to omit references for sake of space limitations.

Papers with more than 14 pages (excluding references) will be rejected without review.
This includes papers where the margins and formatting including the font are deemed to have been significantly altered from those laid down by this style guide.

The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts. 
The reviewing process cannot determine the suitability of the paper for presentation in 14 pages if it is reviewed in 16.


\subsection{Paper ID}
It is imperative that the paper ID is mentioned on each page of the manuscript of the review version.
Enter your paper ID in the appropriate place in the \LaTeX{} template (see \texttt{\%TODO REVIEW}).
The paper ID is a number automatically assigned to your submission when registering your paper submission on the submission site.


\subsection{Line Numbering}
\label{sec:line-numbering}
All lines should be numbered in the initial submission, as in this example document. 
This makes reviewing more efficient, because reviewers can refer to a line on a page. 
Line numbering is removed in the camera-ready version.


\section{Policies}
The policies governing the review process of ECCV \ECCVyear{} are detailed on the conference webpage (see \url{https://eccv2024.ecva.net/}), such as regarding confidentiality, dual submissions, double-blind reviewing, plagiarism, and more. 
By submitting a paper to ECCV, the authors acknowledge that they have read the submission policies and that the submission follows the rules set forth.

Accepted papers will be published in LNCS proceedings with Springer.
To that end, authors must follow the Springer Nature Code of Conduct for Authors (see \url{https://www.springernature.com/gp/authors/book-authors-code-of-conduct}).
We would like to draw particular attention to the policies regarding figures and illustrations, as well as ethical approval and informed consent, which are also reproduced on the ECCV website.


\section{Preserving Anonymity}
\label{sec:blind}
ECCV reviewing is double blind, in that authors do not know the names of the area chair/reviewers of their papers, and the area chairs/reviewers cannot, beyond reasonable doubt, infer the names of the authors from the submission and the additional material. 
You must not identify the authors nor provide links to websites that identify the authors, neither in the paper nor in the supplemental material.
If you need to cite a different paper of yours that is being submitted concurrently to ECCV, you should \emph{(1)} cite these papers anonymously, \emph{(2)} argue in the body of your paper why your ECCV paper is non-trivially different from these concurrent submissions, and \emph{(3)} include anonymized versions of those papers in the supplemental material.
Violation of any of these guidelines may lead to rejection without review. 

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
  \begin{center}
      An analysis of the frobnicatable foo filter.
  \end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}

An example of an acceptable paper:
\begin{quote}
  \begin{center}
     An analysis of the frobnicatable foo filter.
  \end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission [1] as supplemental material and cite it as
\begin{quote}
  [1] Authors. ``The frobnicatable foo filter'', ECCV \ECCVyear Submission ID 00324, Supplied as supplemental material {\tt 00324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not \emph{require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Anonymous24b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem, which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the ECCV audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.

For sake of anonymity, authors must omit acknowledgements in the review copy. 
They can be added later when you prepare the final copy.


\section{Formatting Guidelines}

\subsection{Headings}
Headings should be capitalized (\ie, nouns, verbs, and all other words except articles, prepositions, and conjunctions should be set with an initial capital) and should, with the exception of the title, be aligned to the left.
Only the first two levels of section headings should be numbered, as shown in \cref{tab:headings}.
The respective font sizes are also given in \cref{tab:headings}. 
Kindly refrain from using ``0'' when numbering your section headings.
Words joined by a hyphen are subject to a special rule. 
If the first word can stand alone, the second word should be capitalized.

\begin{table}[tb]
  \caption{Font sizes of headings. 
    Table captions should always be positioned \emph{above} the tables.
  }
  \label{tab:headings}
  \centering
  \begin{tabular}{@{}lll@{}}
    \toprule
    Heading level & Example & Font size and style\\
    \midrule
    Title (centered)  & {\Large\bf Lecture Notes \dots} & 14 point, bold\\
    1st-level heading & {\large\bf 1 Introduction} & 12 point, bold\\
    2nd-level heading & {\bf 2.1 Printing Area} & 10 point, bold\\
    3rd-level heading & {\bf Headings.} Text follows \dots & 10 point, bold\\
    4th-level heading & {\it Remark.} Text follows \dots & 10 point, italic\\
  \bottomrule
  \end{tabular}
\end{table}

Here are some examples of headings: 
``Criteria to Disprove Context-Freeness of Collage Languages'', ``On Correcting the Intrusion of Tracing Non-deterministic Programs by Software'', ``A User-Friendly and Extendable Data Distribution System'', ``Multi-flip Networks: Parallelizing GenSAT'', ``Self-determinations of Man''.


\subsection{Figures}
\label{sect:figures}
For \LaTeX{} users, we recommend integrating figures in your paper using the package \texttt{graphicx}.

It is essential that all illustrations are clear and legible. 
Vector graphics (rather than rasterized images) should be used for diagrams and schemas whenever possible. 
Please check that the lines in line drawings are not interrupted and have a constant width. 
Line drawings are to have a resolution of at least 800 dpi (preferably 1200 dpi).
Grids and details within figures must be clearly legible and may not be written one on top of the other. 
The lettering in figures should not use font sizes smaller than 6\:pt ($\sim$2\:mm character height). 

Figures should be numbered and should have a caption, which should always be positioned \emph{under} the figures, in contrast to the caption belonging to a table, which should always appear \emph{above} the table.
Figures and Tables should be cross-referred in the text.

If they are short, they are centered between the margins (\cf \cref{fig:short}). 
Longer captions, covering more than one line, are justified (\cref{fig:example} shows an example). 
Captions that do not constitute a full sentence, do not have a period.


\begin{figure}[tb]
  \centering
  \includegraphics[height=6.5cm]{eijkel2}
  \caption{One kernel at $x_s$ (\emph{dotted kernel}) or two kernels at $x_i$ and $x_j$ (\emph{left and right}) lead to the same summed estimate at $x_s$.
    This shows a figure consisting of different types of lines.
    Elements of the figure described in the caption should be set in italics, in parentheses, as shown in this sample caption. 
    The last sentence of a figure caption should generally end with a full stop, except when the caption is not a full sentence.
  }
  \label{fig:example}
\end{figure}

\begin{figure}[tb]
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Centered, short example caption}
  \label{fig:short}
\end{figure}

If possible (\eg, if you use \LaTeX) please define figures as floating objects. 
\LaTeX{} users, please avoid using the location parameter ``h'' for ``here''. 
If you have to insert a pagebreak before a figure, please ensure that the previous page is completely filled.


\subsection{Formulas}
Displayed equations or formulas are centered and set on a separate line (with an extra line or half line space above and below). 
Equations should be numbered for reference. 
The numbers should be consecutive within the contribution, with numbers enclosed in parentheses and set on the right margin.
For example,
\begin{align}
  \psi (u) & = \int_{0}^{T} \left[\frac{1}{2}
  \left(\Lambda_{0}^{-1} u,u\right) + N^{\ast} (-u)\right] \text{d}t \; \\
& = 0
\end{align}
and 
\begin{equation}
  E = m\cdot c^2.
  \label{eq:important}
\end{equation}
Please do not include section counters in the numbering.

Numbering equations makes reviewing more efficient, because reviewers can refer to a line on a page.  
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{https://doi.org/10.1063/1.2811173}.

% No color equations in Springer publications.
Equations should never be in color and should be punctuated in the same way as ordinary text.
They should not be pasted in as figures.


\subsubsection{Lemmas, Propositions, and Theorems.}
The numbers accorded to lemmas, propositions, and theorems, \etc should appear in consecutive order, starting with Lemma 1. 
Please do not include section counters in the numbering like ``Theorem 1.1''.


\subsection{Footnotes.}
The superscript numeral used to refer to a footnote appears in the text either directly after the word to be discussed or -- in relation to a phrase or a sentence -- following the punctuation mark (comma, semicolon, or period).%
\footnote{The footnote numeral is set flush left and the text follows with the usual word spacing. 
  Second and subsequent lines are indented. 
}
For remarks pertaining to the title or the authors' names, in the header of a paper, symbols should be used instead of a number.
Please note that no footnotes may be included in the abstract.


\subsection{Cross References}
For the benefit of author(s) and readers, please use the
\begin{verbatim}
  \cref{...}
\end{verbatim}
command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:example} and \cref{tab:headings}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:example,fig:short-a}.
  You may also return to \cref{sec:intro} or look at \cref{eq:important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
\begin{verbatim}
  \Cref{...}
\end{verbatim}
command. Here is an example:
\begin{quotation}
  \Cref{fig:example} is also quite important.
\end{quotation}


\subsection{Program Code}
Program listings or program commands in the text are normally set in typewriter font (\eg, \texttt{printf("Hello world!\textbackslash{}n");}).


\subsection{Citations}
Arabic numbers are used for citation, which is sequential either by order of citation or by alphabetical order of the references, depending on which sequence is used in the list of references. 
The reference numbers are given in brackets and are not superscript.
Please observe the following guidelines:
\begin{itemize}
\item Single citation: \cite{Anonymous24}
\item Multiple citation: \cite{Alpher02,Alpher03,Alpher05,Anonymous24b,Anonymous24}. 
  The numbers should be listed in numerical order.
  If you use the template as advised, this will be taken care of automatically.
\item If an author's name is used in the text: Alpher \cite{Alpher02} was the first \ldots
\end{itemize}
Please write all references using the Latin alphabet. If the title of the book you are referring to is, \eg, in Russian or Chinese, then please write (in Russian) or (in Chinese) at the end of the transcript or translation of the title.
All references cited in the text should be in the list of references and vice versa.

References should be formatted with the official LNCS reference style.
The \LaTeX{} template already takes care of that through the use of the \texttt{splncs04.bst} Bib\TeX{} style file.
Springer strongly encourages you to include DOIs (Digital Object Identifiers) in your references (\cf \cite{ECCV2022}). 
The DOI is a unique code allotted by the publisher to each online paper or journal article. 
It provides a stable way of finding published papers and their metadata. 
The insertion of DOIs increases the overall length of the references section, but this should not concern you as the reference section is not counted toward the page limit.


\subsection{Miscellaneous}
Compare the following:
\begin{center}
  \begin{tabular}{ll}
    \verb'$conf_a$'          & $\qquad conf_a$ \\
    \verb'$\mathit{conf}_a$' & $\qquad \mathit{conf}_a$
  \end{tabular}
\end{center}
See The \TeX book, p.\ 165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, \emph{e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', 
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et\hskip 0.1em}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


\section{Camera-Ready Manuscript Preparation}
\label{sec:manuscript}
This information will follow after paper decisions have been announced.


\section{Conclusion}
The paper ends with a conclusion. 

\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript. This is the last page.
\par\vfill\par
Now we have reached the maximum length of an ECCV \ECCVyear{} submission (excluding references).
References should start immediately after the main text, but can continue past p.\ 14 if needed.
\clearpage  % TODO REVIEW/FINAL: This \clearpage needs to be removed from both review and camera-ready versions.


==> eccv_2024/julia_rebuttal_text.tex <==

\cite{grabinski2022frequencylowcut}
\noindent\textbf{R\#3} Thank you for the constructive and extensive review. We address your questions in the following.

\noindent\emph{ a)Motivation of using adversarial attacks for dense regression tasks (e.g. segmentation, image enhancement, etc.) and why it is more important than clean performance on the main task. b) the hypothesis needs to be validated in both ways (improves the robustness and thus is actually useful for the task)}
\textcolor{orange}{a) Discuss Table 1 in-depth b) as well as Table 4, Figure 5, Figure 7}

\noindent\emph{Space and time complexity}
\textcolor{orange}{ Calculation of number of learnable parameters, time for one epoch average over 10 epochs}

\noindent\emph{Following line 124}
\textcolor{orange}{This should indicate "In the following".}


%\noindent\emph{My fundamental issue with this work is on the usage of adversarial robustness as an evaluation metric. It's not immediately clear why the authors are using robustness to adversarial attacks as a performance metric. The authors state “The purpose of adversarial attacks is to reveal neural networks’ weaknesses [2, 26, 66, 72] by perturbing pixel values in the input image”. Following the author’s argument, then improving adversarial robustness would necessarily improve main task performance, since we’ve identified and addressed the model’s weaknesses. However, the main table 1 very clearly shows that using PixelShuffle and TransposedConv are better for the actual task (image restoration). What is the point of improving adversarial robustness for these types of tasks, i.e. there’s a clear difference between attacking a classifier vs. an image restoration or image segmentation model. The authors state “However, we observe on increasing context 282 283 by increasing the kernel size to 7×7 that the performance of the transposed convolu tion variants significantly improves, especially making the networks more stable when facing adversarial attacks. This boost in performance is further accentuated by increasing the kernel size to 11×11 (both with parallel small kernels).” Sure, you’ve improved the “stability” of the features, but you did not improve the main task performance, so what is the point?
%Moreover, the proposed method does not actually completely defend against the adversarial attack, as is clearly demonstrated in Figure 5. Those are still “attacked” images and not actually enhanced. I understand that the goal is not to actually solve the adversarial attack problem, and instead use it to validate the hypothesis but the hypothesis needs to be validated in both ways (improves the robustness and thus is actually useful for the task). I observe the same issue with Table 4. Following this issue, if we are to consider Figure 7, we can see that on a clean image, the kernel size doesn’t affect the task performance. Even for minimally attacked scenarios (FGSM lines), the kernel size very minimally affects the task performance. I would appreciate it the authors explain this reasoning.
%More discussion is needed on the space and time complexity introduced by increasing the kernel size. Propose larger kerels, the first question is what tradeoff did this introduce? Space (network size, and time, larger number of parameters?)
%Line 124 “Following” what?}


%\noindent\emph{The analysis covers three types of models, this is beneficial and important. My main issue is the usage of adversarial robustness for dense regression tasks (e.g. segmentation, image enhancement, etc.). Please clarify in what scenario this is more relevant than the task performance. For ex, in image classification, less robust means less accurate. In this scenario, your table 1 shows that less robust does not necessarily mean less accurate. Or that increasing robustness necessarily increases task performance.}

\noindent\textbf{R\#4} Thank you for the constructive and extensive review. We address your questions in the following.

\noindent\emph{1. Since the experiments shown in the paper didn’t change the encoder design, the decoder upsampling blocks achieve a specific upsampling factor (let’s say nX). That means when the paper shows the results of the baseline (e.g., in Table 2, 2x2), the used kernel is 2x2 with a stride step of n. Typically in U-Net-like models, n<=4 (upsampling factor <=4X). Then, when the paper reports the results of using a 7x7 kernel (the proposed LCTC), the used stride remains nxn (where n<=4) to achieve the same upsampling factor. This approach may cause grid-like artifacts, as mentioned in Line 81: "If the stride is smaller than the kernel size, this will cause overlaps in the operation, leading to uneven contributions to different pixels in the upsampled feature map and thus to grid-like artifacts." While the paper admits that the performance metrics in the paper do not completely consider spectral artifacts (Line 404), it also states (in the same paragraph) that "Ideally, we would want infinitely large kernels." This statement and the experiments don't align well with the statement in Line 81.}
\textcolor{orange}{TODO}

\noindent\emph{2. The significant drop in performance of the Restormer model using a 3x3 transposed convolution kernel (9.68 PSNR vs. 29.51 using a 7x7 kernel) requires further discussion. It is unclear why changing the kernel size would lead to such a substantial drop in accuracy (almost 20 PSNR). This discrepancy is also apparent in the results under adversarial attacks, where all versions dropped by over 50\% of the original accuracy except for the 3x3 transposed convolution, which only dropped by ~15\%. Additionally, the results in Tables 2-4 for semantic segmentation using a 2x2 kernel show reasonable differences in accuracy (same for Table 6 with 3x3), suggesting that changing the kernel size should not lead to such a significant drop as seen in Table 1.}
\textcolor{orange}{TODO}

\noindent\emph{3. Hypotheses 1 and 2 appear to refer to the same concept: that large kernel sizes in transposed convolution provide more context and reduce spectral artifacts. Hypothesis 2 adds that enlarging the kernel size of non-upsampling kernels will not help, which seems intuitive. While experiments to validate that the improvement doesn't come from increasing learnable parameters are valuable, it might not be necessary to classify them as separate hypotheses.}
\textcolor{orange}{TODO}

\noindent\emph{4. The paper's contributions (Section 1) could be summarized into a single point, avoiding repetition of the same idea.}
\textcolor{orange}{Thank you for reading the paper, we decrease the repetitions and plan to remove lines INSERTE HERE}


\noindent\emph{5. The paper states that the default upsampling factor in CCNs is 2 (Line 134). However, based on the best of my knowledge, there is no “default” upsampling factor in CCNs.}
\textcolor{orange}{TODO}


\noindent\emph{6. The paper refers to bed of nails upsampling as "bed of nails interpolation" (Line 126, 137). However, bed of nails upsampling, as described in Ref [19] and other recommended citations, only inputs one of the input elements in each region, setting the rest to zero, meaning there is no interpolation.
** Additional references **
+ Learning to Generate Chairs, Tables, and Cars with Convolutional Networks. TPAMI, 2016
+ Inverting Visual Representations with Convolutional Networks. In CVPR, 2016
+ Generating Images with Perceptual Similarity Metrics based on Deep Networks. In NeurIPS 2016.}
\textcolor{orange}{TODO}

\noindent\emph{7. The paper states that the resulting interpolated signal by linear interpolation is suboptimal for several reasons (Line 156) without detailing these reasons. For completeness, it is recommended to discuss these reasons further.}
\textcolor{orange}{TODO}


\textbf{ADDITIONS to be changed}

\noindent\emph{- The sentence in Line 35: "anti-aliasing (blurring)" and in Line 96: "While during encoding, artifacts can be reduced by blurring" may be confusing. While some anti-aliasing techniques might involve blurring, it may confuse the reader to equate anti-aliasing with blurring. Anti-aliasing involves blurring in the sense that it often employs a low-pass filter, which attenuates or removes high-frequency components from a signal before it is sampled. However, it's important to note that the goal of anti-aliasing is not specifically to blur the signal, but rather to prevent aliasing artifacts while maintaining the fidelity of the original signal as much as possible.}
\textcolor{orange}{TODO}

\noindent\emph{Polishing our paper:}
\textcolor{orange}{Thank you, for reading our paper in-depth, we appreciate your suggestions and will address all typos, fix the references, capitalization, equations, introduce all abbreviation, adapt the order of our Figures and aggregate Tables 7 and 8 from the appendix to plots.}


% - The reference format is inconsistent; for example: Ref [1]: "Proceedings of the IEEE/CVF International Conference on Computer Vision" vs Ref [5]: "The IEEE Conference on Computer Vision and Pattern 425 426 Recognition (CVPR)".

% - Abbreviations in reference titles should remain capitalized. For example: Ref [2]: Cospgd -> CosPGD, Ref [19]: Cnn -> CNN, and Ref [22]: Swagan -> SWAGAN.

% - Figures should be ordered based on the mention order in the main text. Figure 3 was mentioned before Figure 2.

% - The full name should be mentioned before introducing any abbreviation in the paper, for example (in Line 252) SotA should be state-of-the-art (SotA).

% - It is uncommon to see plain English with spaces in mathematical equations; for example, in Eq. 4 (supplemental materials): $\text {2D Frequency Spectra} = \frac {1}{C}\sum _{c\in C}FFT(x^{pred}_c - x^{gt}_c)$.

% - Tables 7 and 8 in the supplementary materials are difficult for comparisons. It is highly recommended to consider plotting the results in a bar graph or any other visualization for better and easier comparisons.



\noindent\textbf{R\#5} Thank you for the positive review. We address all remaining questions in the following.

\noindent\emph{1. Motivation of using adversarial attacks.}
\textcolor{orange}{TODO}

\noindent\emph{2. In what scenarios will Spectral Artifacts happen?. (Real World)}
%2. A few more real-world examples could be added. Also, in what scenarios will Spectral Artifacts happen? For example, in Baseline method of Fig.1, obvious spatial dependence on the scene object can be observed. Yet, it is not so for the other methods. Is there any intuitive explanation?
\textcolor{orange}{TODO}


\noindent\emph{3. It seems that large kernels are widely used in image classification but don't align well with Hypotheses 1 and 2. Is there any comment on this?}
\textcolor{orange}{TODO}


==> eccv_2024/tables/image_denoising.tex <==
\begin{table*}[ht]
\caption{ Image Denoising on SSID dataset using NAFNet}
\label{tbl:ablation:image_denoising}
\centering
%\tiny
\scalebox{0.73}{
%\Rotatebox{90}{%
\begin{tabular}{@{}p{1.5cm} c@{\hspace{0.5cm}} c @{\hspace{0.1cm}} c @{\hspace{0.5cm}} | c @{\hspace{0.1cm}} c @{\hspace{0.1cm}} c @{\hspace{0.1cm}} c @{\hspace{0.1cm}} c @{\hspace{0.1cm}} c   @{\hspace{0.5cm}} | c @{\hspace{0.1cm}} c @{\hspace{0.1cm}} c @{\hspace{0.1cm}} c @{\hspace{0.1cm}} c @{\hspace{0.1cm}} c @{}}
\toprule
\multirow{3}{1.5cm}{\textbf{Network}} & \multirow{3}{*}{\textbf{Upsampling Method}} & \multicolumn{2}{c}{\textbf{Test Accuracy}}   & \multicolumn{6}{c}{\textbf{CosPGD attack iterations}} &  \multicolumn{6}{c}{\textbf{PGD attack iterations}} \\
  &  & &  & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{20}   & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{20}                                  \\
& &  PSNR & SSIM &  PSNR & SSIM &  PSNR & SSIM &  PSNR & SSIM &  PSNR & SSIM &  PSNR & SSIM &  PSNR & SSIM \\
\midrule

\iffalse
\multirow{4}{*}{Restormer} & Pixel Shuffle &  \\

& Transposed Conv 3$\times$3 &   \\

& Transposed Conv 7$\times$7 + 3 $\times$3 (Ours) &  \\

& Transposed Conv 11$\times$11 + 3$\times$3 (Ours) &  \\

\midrule
\fi

\multirow{4}{*}{NAFNet} & Pixel Shuffle & 39.97 & 0.9599 & 29.56 & 0.8528 & 28.73 & 0.8307 & 28.25 & 0.8089 & 29.56 & 0.8528 & 28.73 & 0.8308 & 28.26 & 0.8093 \\

& Transposed Conv 3$\times$3 & 39.64 & 0.9581 & 27.09 & 0.7654 & 25.67 & 0.7216 & 24.73 & 0.6891 & 27.09 & 0.7654 & 25.67 & 0.7206 & 24.88 & 0.6922  \\

& Transposed Conv 7$\times$7 + 3 $\times$3 (Ours) & 39.72 & 0.9585 & 29.29 & 0.8331 & 28.34 & 0.8 & 27.64 & 0.77 & 29.29 & 0.83 & 28.31 & 0.8 & 27.65 & 0.77 \\

& Transposed Conv 11$\times$11 + 3$\times$3 (Ours) & 39.70 & 0.9584 & 29.05 & 0.819 & 27.83 & 0.7657 & 26.58 & 0.695 & 29.05 & 0.819 & 27.82 & 0.7649 & 26.59 & 0.6952 \\

\midrule
\multicolumn{16}{c}{After Adversarial Training} \\
\midrule

\multirow{4}{*}{NAFNet} & Pixel Shuffle & 39.73 & 0.9584 & 28.07 & 0.7582 & 26.53 & 0.7018 & 24.0 & 0.6136 & 28.06 & 0.7579 & 26.49 & 0.7002 & 23.95 & 0.6105  \\

& Transposed Conv 3$\times$3 & 39.65 & 0.958 & 28.19 & 0.768 & 27.15 & 0.7273 & 26.35 & 0.6959 & 28.19 & 0.7682 & 27.16 & 0.7279 & 26.33 & 0.6942 \\

& Transposed Conv 7$\times$7 + 3 $\times$3 (Ours) & 39.69 & 0.9582 & 27.9 & 0.7406 & 26.79 & 0.6931 & 25.74 & 0.6527 & 27.9 & 0.7404 & 26.78 & 0.6945 & 25.74 & 0.6530  \\

& Transposed Conv 11$\times$11 + 3$\times$3 (Ours) & 39.7 & 0.9583 & 27.66 & 0.727 & 26.67 & 0.6818 & 25.79 & 0.6422 & 27.66 & 0.7273 & 26.66 & 0.6796 & 25.75 & 0.639  \\

\bottomrule

\end{tabular}
}
\end{table*}

==> eccv_2024/tables/kernel_limit_all.tex <==
\begin{table*}[t]
\caption{Comparison of performance of very large: 31$\times$31 kernels in transposed convolution to large kernels (7$\times$7 to 11$\times$11). 
We additionally test with medium-size kernels~(5$\times$5) as a parallel kernel to the large kernels instead of 3$\times$3.
Here we observe the saturation of performance for very large kernels for upsampling. 
This comparison is for the same encoder and the same ResNet-like building blocks in the decoder.
}
\label{tbl:appendix:kernel_limit_all}
\centering
%\tiny
\scalebox{.71}{
\begin{tabular}{p{3cm}ccc|ccc|ccc|ccc|ccc}
\toprule
 \multirow{3}{3cm}{\textbf{Transposed Convolution Kernels}} & \multicolumn{3}{c}{\textbf{Test Accuracy}} & \multicolumn{9}{c}{\textbf{FGSM attack epsilon}} & \multicolumn{3}{c}{\textbf{SegPGD attack iterations}} \\
& \multirow{2}{*}{mIoU} & \multirow{2}{*}{mAcc} & \multirow{2}{*}{allAcc} & \multicolumn{3}{c}{0.10} & \multicolumn{3}{c}{0.20} & \multicolumn{3}{c}{0.30}  &  \multicolumn{3}{c}{20}  \\
 &   &  &  &  mIoU & mAcc & allAcc & mIoU & mAcc & allAcc & mIoU & mAcc & allAcc & mIoU & mAcc & allAcc\\
\midrule
7$\times$7 & 0.71 & 0.85 & 0.93 & 0.45 & 0.67 & 0.82 & 0.44 & 0.64 & 0.82 & 0.43  & 0.61 & 0.82  & 0.14 & 0.44 & 0.37 \\ 
9$\times$9 & 0.71  & 0.84 & 0.93 &0.46  & 0.69 & 0.82 & 0.45 & 0.65 & 0.83 &  0.42 & 0.60 & 0.81  & 0.15 & 0.47 & 0.39 \\ 
9$\times$9 + 3$\times$3 & 0.72 & 0.85 & 0.93 & 0.46 & 0.68 & 0.83 & 0.45 & 0.66 & 0.82 &  0.43 & 0.62 &  0.81 & 0.14 & 0.46 & 0.35 \\ 
11$\times$11 + 3$\times$3 &  0.72 & 0.85 & 0.93 & 0.47 & 0.70 & 0.83  & 0.45 & 0.65 & 0.82 &  \textbf{0.44} & 0.63 & \textbf{0.83}  &    \textbf{0.16} & 0.48 & 0.39 \\
 15$\times$15 + 3$\times$3 & \textbf{0.73} & \textbf{0.86} & 0.93 & 0.47 & 0.70 & 0.83 & 0.46 & 0.67 & 0.82 & 0.44  & 0.63 & 0.82  & 0.15 & 0.47 & 0.37 \\ 
 17$\times$17 + 3$\times$3 & 0.72 & 0.85 & 0.93 & 0.47 & 0.70 & 0.83 & \textbf{0.46} & \textbf{0.67} & \textbf{0.83} &  0.44 & \textbf{0.64} & 0.82  & 0.15 & \textbf{0.49} & 0.36 \\ 
 31$\times$31 + 3$\times$3 &  0.71 & 0.85 & 0.93 &  0.47 & 0.68 & 0.83 & 0.45 & 0.65 & 0.82 & 0.43 & 0.60 & 0.82 & 0.15 & 0.44 & 0.41\\
 31$\times$31 + 5$\times$5 &  0.71 & 0.85 & 0.93 &  0.46 & 0.67 & 0.83 & 0.45 & 0.65 & 0.82 & 0.43 & 0.61 & 0.82 & 0.15 & 0.44 & 0.41\\
\bottomrule

\end{tabular}
}
\end{table*}

==> eccv_2024/tables/nafnet_ood_perf.tex <==
\begin{table}[t]
    \centering
    %\vspace{0em}
    %\scriptsize
    %    
    % 
    \caption{Performance of different upsampling methods in NAFNet in real-world ODD setting by applying 2D common corruption\cite{commoncorruptions} (severity=3) on GoPro dataset. We use all common corruptions from \cite{commoncorruptions} GitHub repository except weather conditions (ideally these should happen before the motion blurring) and blurring (since the images are already motion blurred). Here ``Mean'' is performance over all the considered corruptions:}
    \scalebox{0.8}{
    \begin{tabular}{@{}c@{\hspace{0.3cm}}|@{\hspace{0.3cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{}c@{}c@{\hspace{0.2cm}}c@{}}
        %\multirow{2}{*}{Upsampling Method} 
        \toprule
        Upsampling Method & \multicolumn{2}{c@{\hspace{0.2cm}}}{Shot Noise} & \multicolumn{2}{@{\hspace{-0.1cm}}c}{JPEG Compression} & \multicolumn{2}{c}{Mean} \\
       & { PSNR} & { SSIM} & { PSNR} & { SSIM} & { PSNR} & { SSIM} \\
        \midrule
        %\hline
        Pixel Shuffle  & 4.86 & 0.0127 & 25.28 & 0.8095 & 15.84 & 0.4447 \\
        Trans.~Conv.~3$\times$3  & 8.95 & 0.0984 & 25.10  & 0.8032 & 17.28 & 0.4798 \\
        % LCTC 7$\times$7+3$\times$3 &  & \\
        LCTC 11$\times$11+3$\times$3  & \textbf{13.25} & \textbf{0.1564} & \textbf{25.38} & \textbf{0.8104} & \textbf{19.26} & \textbf{0.5127}  \\
    \bottomrule
    \end{tabular}    
    }
    \label{tab:ood_nafnet}
    %\vspace{-2.8em}
\end{table}

==> eccv_2024/tables/seg_clean_acc.tex <==
\begin{table}[t]
\caption{Semantic Segmentation performance on the PASCAL VOC2012 validation set for UNet with ConvNeXt encoder, and the baseline UNet decoder (see \Cref{fig:unet_plus_block}) with differently sized \textcolor{BrickRed}{kernels in transposed convolution for feature map upscaling}.}
\label{tbl:exp:semantic:unet-convnext-test}
\centering
%\tiny
\scalebox{.63}{
\begin{tabular}{p{5cm}|ccc}
% \toprule
 \multirow{2}{5cm}{\textbf{Transposed Convolution Kernels}}& \multicolumn{3}{c}{\textbf{Test Accuracy}}      \\
  &  mIoU  &  mAcc & allAcc \\
\midrule
 2$\times$2 (baseline) &    78.34 & 86.89 & 95.15  \\
 7$\times$7    &  78.92 & \textbf{88.06} & 95.23   \\
 \textbf{11$\times$11 + 3$\times$3}    &  \textbf{79.33} & 87.81 & \textbf{95.41} \\
% \bottomrule

\end{tabular}
}
\vspace{-1em}
\end{table}

==> eccv_2024/tables/table_from_rebuttal.tex <==
\begin{table}[t]
    \centering
    \vspace{0em}
    %\scriptsize
    %\tiny    
    % 
    \caption{Performance of different upsampling methods in NAFNet in real-world ODD setting by applying 2D common corruption\cite{commoncorruptions} (severity=3) on GoPro dataset. We use all common corruptions from \cite{commoncorruptions} GitHub repository except weather conditions (ideally these should happen before the motion blurring) and blurring (since the images are already motion blurred).Here ``Mean'' is performance over all the considered corruptions:}
    \scalebox{0.8}{
    \begin{tabular}{@{}c@{}c@{\,\,\,}c@{\hspace{0.3cm}}|@{\hspace{0.3cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{}c@{}c@{\hspace{0.2cm}}c@{}}
        %\multirow{2}{*}{Upsampling Method} 
        Upsampling & Latency & No. of & \multicolumn{2}{@{\,\,}c@{\hspace{0.2cm}}}{Shot Noise} & \multicolumn{2}{@{\hspace{-0.1cm}}c}{JPEG Compression} & \multicolumn{2}{c}{Mean} \\
        Method & (ms) & Params. & {\tiny PSNR} & {\tiny SSIM} & {\tiny PSNR} & {\tiny SSIM} & {\tiny PSNR} & {\tiny SSIM} \\
        %\midrule
        \hline
        Pixel Shuffle & 0.26  & 17.11 M & 4.86 & 0.0127 & 25.28 & 0.8095 & 15.84 & 0.4447 \\
        Trans.~Conv.~3$\times$3 & 0.27 & 16.43 M  & 8.95 & 0.0984 & 25.10  & 0.8032 & 17.28 & 0.4798 \\
        % LCTC 7$\times$7+3$\times$3 &  & \\
        LCTC 11$\times$11+3$\times$3 & 0.38 & 16.54 M & \textbf{13.25} & \textbf{0.1564} & \textbf{25.38} & \textbf{0.8104} & \textbf{19.26} & \textbf{0.5127}  \\
    \end{tabular}    
    }
    \label{tab:ood_nafnet}
    %\vspace{-2.8em}
\end{table}
